Zephon: Elastic Determinism for Online, Stateful Foundation Model Data Loading Pipelines

Deterministic data loading is important for foundation model development: model researchers need confidence that differences they observe across costly ablations are caused by the parameter they changed rather than non-determinism in the training data sequence. The data loader must provide elastic determinism, i.e., a deterministic sequence of global training data batches despite changes to the GPU topology across runs (e.g., due to GPU scarcity), frequent checkpoint-resume cycles, and different data processing execution backends. Achieving this is difficult because modern foundation model data pipelines tokenize, pack, and mix samples online, introducing stateful n-to-m transformations that break sample indexing. Existing data loaders largely assume indexable 1-to-1 pipelines, and the common workaround of offline materialization is expensive and, for some modalities such as video, infeasible. We present Zephon, a data loader for foundation models that supports online, stateful pipelines while providing elastic determinism and efficient resumption from checkpoints. It partitions the global stream into topology-independent lanes, serializes ordering decisions while parallelizing stateless work on interchangeable backends, and checkpoints only bounded in-flight state so recovery cost does not grow with training progress. We evaluate Zephon on text and vision-language workloads and show that it achieves competitive throughput while providing a combination of guarantees that no existing loader offers for online, stateful pipelines.

==> meta/commands.tex <==
\settopmatter{authorsperrow=4}

\makeatletter
\patchcmd{\@mkauthors@iii}{\mathchardef\UrlBreakPenalty=10000}{}{}{\message{[zephon] email-break patch 1 FAILED}}
\patchcmd{\@mkauthors@iii}{\mathchardef\UrlBreakPenalty=10000}{}{}{\message{[zephon] email-break patch 2 FAILED}}
\makeatother

\makeatletter
\def\@ACM@checkaffil{}
\makeatother

\makeatletter
\newcount\zephon@acount    \zephon@acount=0
\newcount\zephon@wideuntil \zephon@wideuntil=12  %
\newdimen\zephon@narrowW
\newdimen\zephon@colA \zephon@colA=110pt %
\newdimen\zephon@colB \zephon@colB=92pt  %
\newdimen\zephon@colC \zephon@colC=134pt %
\newdimen\zephon@colD \zephon@colD=110pt %
\AtBeginDocument{%
  \zephon@narrowW=\textwidth \advance\zephon@narrowW by -\author@bx@sep
    \divide\zephon@narrowW by 5 \advance\zephon@narrowW by -\author@bx@sep}
\def\@typeset@author@bx{%
  \global\advance\zephon@acount by 1\relax
  \ifnum\zephon@acount>\zephon@wideuntil\relax
    \author@bx@wd=\zephon@narrowW            %
  \else                                      %
    \@tempcnta=\zephon@acount \advance\@tempcnta by -1
    \@tempcntb=\@tempcnta \divide\@tempcntb by 4 \multiply\@tempcntb by 4
    \advance\@tempcnta by -\@tempcntb           %
    \ifcase\@tempcnta
      \author@bx@wd=\zephon@colA \or
      \author@bx@wd=\zephon@colB \or
      \author@bx@wd=\zephon@colC \or
      \author@bx@wd=\zephon@colD \fi
  \fi
  \bgroup\hsize=\author@bx@wd
    \def\and{\par}\normalbaselines
    \global\setbox\author@bx=\vtop{\if@ACM@sigchiamode\else\centering\fi
      \@authorfont\@currentauthors\par\@affiliationfont
      \@currentaffiliation}%
  \egroup
  \box\author@bx\hspace{\author@bx@sep}%
  \gdef\@currentauthors{}%
  \gdef\@currentaffiliation{}}
\makeatother

\ifluatex
\else
\DeclareUnicodeCharacter{2212}{−}
\fi

\newcommand{\CPP}{C\texttt{++}\xspace}
\newcommand{\cth}{\(c\)\textsuperscript{th}}

\newcommand{\td}[1]{{#1}}
\newcommand{\vldb}[1]{{#1}}
\newcommand{\revi}[1]{{#1}}
\newcommand{\revMRa}[1]{{#1}}
\newcommand{\revMRb}[1]{{#1}}
\newcommand{\revMRc}[1]{{#1}}
\newcommand{\revMRd}[1]{{#1}}
\newcommand{\revMRe}[1]{{#1}}
\newcommand{\revMRf}[1]{{#1}}
\newcommand{\revMRg}[1]{{#1}}
\newcommand{\revMRh}[1]{{#1}}
\newcommand{\revDc}[1]{{#1}}
\newcommand{\revM}[1]{{#1}}
\newcommand{\revSteve}[1]{{#1}}
\newcommand{\varone}[1]{{#1}}
\newcommand{\vartwo}[1]{{#1}}

\newcommand{\fixme}[1]{}
\newcommand{\ana}[1]{}
\newcommand{\maxi}[1]{}
\newcommand{\ties}[1]{}
\newcommand{\xianz}[1]{}


\newcommand*{\mixtera}{\texorpdfstring{\dynamicwidth{\textsc{Mixtera}}{\textsc{Mixtera}}}{Mixtera}}
\newcommand*{\omlette}{\mixtera} %

\newcommand*{\zephon}{\texorpdfstring{\dynamicwidth{\textsc{Zephon}}{\textsc{Zephon}}}{Zephon}}


\definecolor{LightGray}{gray}{0.95}



\hyphenation{Data-Loader}



\definecolor{plotorange}{rgb}{0.8705882352941177, 0.5607843137254902, 0.0196078431372549}
\definecolor{plotred}{rgb}{0.8115340253748559, 0.3211072664359862, 0.2758169934640523}
\definecolor{plotblue}{rgb}{0.2366013071895425, 0.5418685121107266, 0.7470203767781622}


\DeclareRobustCommand{\mybox}[2][gray!20]{%
\begin{tcolorbox}[   %
        breakable,
        left=0pt,
        right=0pt,
        top=0pt,
        bottom=0pt,
        colback=#1,
        colframe=#1,
        width=\dimexpr\textwidth\relax, 
        enlarge left by=0mm,
        boxsep=5pt,
        arc=0pt,outer arc=0pt,
        ]
        #2
\end{tcolorbox}
}
\newcommand{\kmessage}[1]{%
\begin{tcolorbox}[
    colback=blue!5!white,
    colframe=blue!75!black,
    width=\linewidth,
    left skip=0pt,
    right skip=0pt,
    boxrule=0.5pt,
    left=1mm,
    right=1mm,
    top=1mm,
    bottom=1mm,
    boxsep=1pt,
    arc=0mm,
    before skip=4pt,
    after skip=4pt
]
\small
\textit{Key Message}: #1
\end{tcolorbox}}

\newcommand{\s}[1]{\textsc{#1}}
\newcommand{\z}{\small\scshape}

\newcommand{\na}{\small{\textsc{Z-Proc} \footnotesize{(no GIL)}}}
\newcommand{\nb}{\small{\textsc{Z-Thread} \footnotesize{(no GIL)}}}
\newcommand{\nc}{\small{\textsc{Z-Proc} \footnotesize{(OS Pipe)}}}

